From Evidence to Belief: A Bayesian Epistemology Approach to Language Models

This paper investigates the knowledge of language models from the perspective of Bayesian epistemology. We explore how language models adjust their confidence and responses when presented with evidence with varying levels of informativeness and reliability. To study these properties, we create a dataset with various types of evidence and analyze language models' responses and confidence using verbalized confidence, token probability, and sampling. We observed that language models do not consistently follow Bayesian epistemology: language models follow the Bayesian confirmation assumption well with true evidence but fail to adhere to other Bayesian assumptions when encountering different evidence types. Also, we demonstrated that language models can exhibit high confidence when given strong evidence, but this does not always guarantee high accuracy. Our analysis also reveals that language models are biased toward golden evidence and show varying performance depending on the degree of irrelevance, helping explain why they deviate from Bayesian assumptions.

==> results/gemini_result.tex <==
\begin{table*}[!hbt]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|cccccccc}
\hline
                               & \textbf{Dataset}     &\textbf{Metric}   & \textbf{No\_EVI} & \textbf{EVI}   & \textbf{Coincidence} & \textbf{Irrelevant} & \textbf{Conflict} & \textbf{Incomplete} & \textbf{Contradiction} \\ \hline \hline
\multirow{9}{*}{\textbf{Gemini-1.5-Flash}} & \multirow{3}{*}{SciQ}  & Confidence  & 0.93   & 0.983 & 0.851       & 0.554      & 0.771    & 0.936      & 0.96         \\
                               &                         & Accuracy \(\uparrow\)  & 0.65   & 0.86  & 0.885       & 0.66      & 0.62      & 0.79      & 0.87         \\
                               &                         & ECE  \(\downarrow\)    & 0.28   & 0.123 & 0.082       & 0.263      & 0.218    & 0.146      & 0.09          \\     \cline{2-10} 
                               & \multirow{3}{*}{Trivia} & Confidence             & 0.909   & 0.881  & 0.791    & 0.45      & 0.644    & 0.855      & 0.854         \\
                               &                         & Accuracy \(\uparrow\)  & 0.855   & 0.91 & 0.97       & 0.62      & 0.73    & 0.88      & 0.93         \\
                               &                         & ECE  \(\downarrow\)    & 0.087   & 0.063 & 0.179       & 0.252      & 0.234     & 0.086      & 0.076         \\ \cline{2-10} 
                               & \multirow{3}{*}{GSM8K}  & Confidence             & 0.987   & 1.0   & 0.702    & 0.546      & 0.552    & 0.967       & 0.967         \\
                               &                         & Accuracy \(\uparrow\)  & 0.165    & 0.97 & 0.64       & 0.15      & 0.07    & 0.74      & 0.965         \\
                               &                         & ECE   \(\downarrow\)   & 0.822   & 0.03 & 0.373       & 0.476      & 0.542     & 0.277      & 0.044         \\  \hline

\end{tabular}%

}
\caption{The result of confirmation task with verbal method. We used 200 samples for Gemini-1.5-Flash due to the cost limit.}
\label{tab:Gemini_main_verbal}
\end{table*}



\begin{table*}[!hbt]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|cccccccc}
\hline
                               & \textbf{Dataset}     &\textbf{Metric}   & \textbf{No\_EVI} & \textbf{EVI}   & \textbf{Coincidence} & \textbf{Irrelevant} & \textbf{Conflict} & \textbf{Incomplete} & \textbf{Contradiction} \\ \hline \hline
\multirow{9}{*}{\textbf{Gemini-1.5-Flash}} & \multirow{3}{*}{SciQ}  & Confidence  & 0.9     & 0.965 & 0.954       & 0.864      & 0.907    & 0.942      & 0.963         \\
                               &                         & Accuracy \(\uparrow\)  & 0.665   & 0.895 & 0.91       & 0.57     & 0.58     & 0.795      & 0.89         \\
                               &                         & ECE  \(\downarrow\)    & 0.335   & 0.105 & 0.09       & 0.43      & 0.42    & 0.205      & 0.11          \\     \cline{2-10} 
                               & \multirow{3}{*}{Trivia} & Confidence             & 0.882   & 0.964 & 0.971     & 0.882      & 0.915    & 0.95      & 0.96         \\
                               &                         & Accuracy \(\uparrow\)  & 0.838   & 0.905 & 0.97       & 0.593      & 0.65    & 0.839      & 0.9         \\
                               &                         & ECE  \(\downarrow\)    & 0.162   & 0.095 & 0.03       & 0.407      & 0.35     & 0.161      & 0.1         \\ \cline{2-10} 
                               & \multirow{3}{*}{GSM8K}  & Confidence             & 0.826   & 0.99  & 0.962    & 0.818      & 0.907    & 0.954       & 0.989         \\
                               &                         & Accuracy \(\uparrow\)  & 0.19    & 0.97 & 0.64       & 0.14      & 0.055    & 0.715      & 0.965         \\
                               &                         & ECE   \(\downarrow\)   & 0.81   & 0.03  & 0.356       & 0.859      & 0.945     & 0.285      & 0.035         \\  \hline

\end{tabular}%

}
\caption{The result of confirmation task with token probability method. We used 200 samples for Gemini-1.5-Flash due to the cost limit.}
\label{tab:Gemini_main_token}
\end{table*}



\begin{table*}[!hbt]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|cccccccc}
\hline
                               & \textbf{Dataset}     &\textbf{Metric}   & \textbf{No\_EVI} & \textbf{EVI}   & \textbf{Coincidence} & \textbf{Irrelevant} & \textbf{Conflict} & \textbf{Incomplete} & \textbf{Contradiction} \\ \hline \hline
\multirow{9}{*}{\textbf{Gemini-1.5-Flash}} & \multirow{3}{*}{SciQ}  & Confidence  & 0.952   & 0.991 & 0.987       & 0.91      & 0.955    & 0.98      & 0.992         \\
                               &                         & Accuracy \(\uparrow\)  & 0.656   & 0.898 & 0.911       & 0.57      & 0.617      & 0.799      & 0.904         \\
                               &                         & ECE  \(\downarrow\)    & 0.294   & 0.107 & 0.081       & 0.339      & 0.337    & 0.186      & 0.09          \\     \cline{2-10} 
                               & \multirow{3}{*}{Trivia} & Confidence             & 0.929   & 0.969  & 0.929    & 0.885      & 0.907    & 0.969      & 0.99         \\
                               &                         & Accuracy \(\uparrow\)  & 0.839   & 0.894 & 0.839      & 0.599      & 0.658    & 0.84      & 0.894         \\
                               &                         & ECE  \(\downarrow\)    & 0.11    & 0.076 & 0.11       & 0.293      & 0.248     & 0.134      & 0.096         \\ \cline{2-10} 
                               & \multirow{3}{*}{GSM8K}  & Confidence             & 0.72    & 0.996  & 0.947    & 0.705     & 0.852    & 0.936       & 0.994         \\
                               &                         & Accuracy \(\uparrow\)  & 0.19    & 0.97 & 0.633      & 0.151     & 0.061    & 0.721      & 0.97         \\
                               &                         & ECE   \(\downarrow\)   & 0.53   & 0.034 & 0.314       & 0.554      & 0.791     & 0.215      & 0.032         \\  \hline

\end{tabular}%

}
\caption{The result of confirmation task with sampling method. We used 200 samples for Gemini-1.5-Flash due to the cost limit.}
\label{tab:Gemini_main_sampling}
\end{table*}









\begin{table*}[!hbt]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|ccccccccc}
\hline
                               & \textbf{Dataset}     &\textbf{Metric}   & \textbf{High Source} & \textbf{Low Source}   & \textbf{High Spec} & \textbf{Low Spec} & \textbf{Recent} & \textbf{Old} & \textbf{Experiment} & \textbf{Observation} \\ \hline \hline
\multirow{9}{*}{\textbf{Gemini-1.5-Flash}} & \multirow{3}{*}{SciQ}  & Confidence  & 0.981   & 0.822 & 0.976       & 0.944      & 0.965    & 0.917      & 0.974   &0.933      \\
                               &                         & Accuracy \(\uparrow\)  & 0.865   & 0.855 & 0.795       & 0.87       & 0.86     & 0.76       & 0.83     &0.785     \\
                               &                         & ECE  \(\downarrow\)    & 0.119   & 0.065 & 0.181       & 0.084      & 0.105    & 0.168      & 0.158   &0.148         \\     \c      \\  \hline

\end{tabular}%

}
\caption{The result of the strength of evidence task with the verbal method. We used 200 samples for Gemini-1.5-Flash due to the cost limit.}
\label{tab:Gemini_str_verbal}
\end{table*}




\begin{table*}[!hbt]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|ccccccccc}
\hline
                               & \textbf{Dataset}     &\textbf{Metric}   & \textbf{High Source} & \textbf{Low Source}   & \textbf{High Spec} & \textbf{Low Spec} & \textbf{Recent} & \textbf{Old} & \textbf{Experiment} & \textbf{Observation} \\ \hline \hline
\multirow{9}{*}{\textbf{Gemini-1.5-Flash}} & \multirow{3}{*}{SciQ}  & Confidence  & 0.944   & 0.955 & 0.947     & 0.942     & 0.944    & 0.936      & 0.942   &0.955      \\
                               &                         & Accuracy \(\uparrow\)  & 0.855   & 0.855 & 0.8       & 0.85      & 0.88     & 0.76       & 0.835     &0.81     \\
                               &                         & ECE  \(\downarrow\)    & 0.145   & 0.145 & 0.2       & 0.15      & 0.12    & 0.24      & 0.165   &0.19         \\     \c      \\  \hline

\end{tabular}%

}
\caption{The result of the strength of evidence task with the token probability method. We used 200 samples for Gemini-1.5-Flash due to the cost limit.}
\label{tab:Gemini_str_token}
\end{table*}


\begin{table*}[!hbt]
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|c|ccccccccc}
\hline
                               & \textbf{Dataset}     &\textbf{Metric}   & \textbf{High Source} & \textbf{Low Source}   & \textbf{High Spec} & \textbf{Low Spec} & \textbf{Recent} & \textbf{Old} & \textbf{Experiment} & \textbf{Observation} \\ \hline \hline
\multirow{9}{*}{\textbf{Gemini-1.5-Flash}} & \multirow{3}{*}{SciQ}  & Confidence  & 0.974   & 0.986 & 0.978       & 0.981      & 0.97     & 0.964      & 0.973   &0.982      \\
                               &                         & Accuracy \(\uparrow\)  & 0.879   & 0.854 & 0.809       & 0.853      & 0.879     & 0.774       & 0.83     &0.791     \\
                               &                         & ECE  \(\downarrow\)    & 0.106   & 0.133 & 0.169       & 0.128      & 0.091    & 0.193      & 0.15   &0.193         \\     \c      \\  \hline

\end{tabular}%

}
\caption{The result of the strength of evidence task with the sampling method. We used 200 samples for Gemini-1.5-Flash due to the cost limit.}
\label{tab:Gemini_str_samplin}
\end{table*}
